Aspects of entanglement with background electric and magnetic fields in quantum field theoretic systems

This thesis investigates the impact of the background magnetic field on correlations or entanglement between pairs created by the background electric field in quantum field theoretic systems in the Minkowski, the primordial inflationary de Sitter and the Rindler spacetimes. These analyses might provide insight into the relativistic entanglement in the early inflationary universe scenario, where such background fields might exist due to primordial fluctuations, and in the near-horizon of non-extremal black holes, which are often endowed with background electromagnetic fields due to the accretion of plasma onto them.

==> title_first.tex <==
\begin{titlepage}

\begin{center}
%\vspace*{0.25in}

%{
    %\fontencoding{OT1}
   % \fontfamily{ppl}
    %\fontseries{b}
    %\fontshape{sc}
   % \fontsize{22}{40}
    %\fontsize{22}{}
    %\selectfont
   \textbf{\Large Thesis title goes here}\\
%}




\vspace*{2in}



%\vspace*{0.25in}

\textbf{\large \bf Shinki}\\
%\textbf{DEPARTMENT OF PHYSICS}
%\\Indian Institute of Technology Ropar\\for the
%degree of\\Doctor of Philosophy (Science)\\in Physics}


\vspace*{2in}

\begin{figure}[h!]
 \begin{center}
  \includegraphics[width=4cm]{logo.jpg}
 \end{center}
\end{figure}


\textbf{DEPARTMENT OF PHYSICS}\\
\normalsize{\textbf{INDIAN INSTITUTE OF TECHNOLOGY ROPAR}}

%\normalsize{\textbf{INDIA}}

\normalsize{\textbf{JULY 2021}}

\end{center}
\end{titlepage}

\thispagestyle{empty}
